Enhancing Android Application Bug Reporting

The modern software development landscape has seen a shift in focus toward mobile applications as smartphones and tablets near ubiquitous adoption. Due to this trend, the complexity of these "apps" has been increasing, making development and maintenance challenging. Current bug tracking systems do not effectively facilitate the creation of bug reports with useful information that will directly lead to a bug's resolution. To address the need for an improved reporting system, we introduce a novel solution, called Fusion, that helps reporters auto-complete reproduction steps in bug reports for mobile apps by taking advantage of their GUI-centric nature. Fusion links information, that reporters provide, to program artifacts extracted through static and dynamic analysis performed beforehand. This allows our system to facilitate the reporting process for developers and testers, while generating more reproducible bug reports with immediately actionable information.

==> ack.tex <==
This work is supported in part by the NSF CCF-1218129 and NSF CCF-1253837 grants.  Any opinions, findings, and conclusions expressed herein are the authors' and do not necessarily reflect those of the sponsors. 


==> limitations.tex <==
Currently, the DFS implementation in FUSION only supports the \textit{click/tap} action.  Another option to gather runtime program information would be to record app scenarios and replay them while collecting program data or using language modeling based approaches for scenario generation \cite{Linares:MSR15} .  However, we forwent these approaches in favor of the fully automatic DFS application exploration.  Part of our immediate plan for future work includes adding support for more gestures to our DFS engine.  FUSION is currently not capable of capturing certain contextual app  information such as a change in device orientation or network state.  However, this can be mitigated by the fact that reporters can enter such contextual information in the free-form text field associated with each step.  FUSION is also limited in the types of bugs that it can report.  For instance, certain performance or energy bugs would not be as useful reported through FUSION, as the steps to reduce for these non-functional types of bugs may not be as well defined as bugs that can be triggered by manipulating GUI components.  Also, FUSION does not perform any analysis on stack traces in order to reverse-engineer reproduction steps, it is purely a mechanism to aid users in reporting functional, and GUI-related bugs.  

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }



\newcommand\MARTY[1]{\nb{MARTY}{#1}}
\newcommand\KEVIN[1]{\nb{KEVIN}{#1}}
\newcommand\DENYS[1]{\nb{DENYS}{#1}}
\newcommand\MARIO[1]{\nb{MARIO}{#1}}
\newcommand\CARLOS[1]{\nb{CARLOS}{#1}}

\newcommand\NEW[1]{\nb{NEW}{#1}}





